Formal Analysis of a Fault-Tolerant Extension of the ROSACE Flight Controller

Autonomous avionics controllers must satisfy stringent real-time functional and performance require- ments even in the presence of run-time faults. In this paper, we analyze ROSACE, an open-source control engineering benchmark for flight control systems, focusing on its run-time resilience against faults such as sensor noise and sensor failures. We extend the benchmark with an FDIR (Fault Detection, Identification and Recovery) component based on Triple Modular Redundancy. Our approach builds upon COMPASTA, a tool for Model-Based Design developed on top of the TASTE tool by ESA. COMPASTA enables the modeling and injection of faults into a system's design. Moreover, it implements a simulation-based verification and validation workflow, automating the generation and execution of a set of test cases, based on a user-defined notion of coverage. Using COMPASTA, we construct a set of formal models, with faults and with FDIR, and we formally analyze their impact on the system properties. The analysis is based on the coupling of the formal models with the Simulink models used for the simulations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{54}
\providecommand{\publicationstatus}{Matt Luckcuck, Maike Schwammberger, \& Akhila Bairy (Eds.):\\
Eighth International Workshop on Formal Methods\\
for Autonomous Systems (FMAS 2026)\\
EPTCS 457, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.457.5}{10.4204/EPTCS.457.5}}
\pdfoutput=1

